A Framework for Joint Affine and Diffeomorphic Image Registration

Anatomical image registration commonly relies on a sequential pipeline where an affine alignment is estimated first and then held fixed while a non-rigid diffeomorphic deformation is applied. This two-step process often leads to suboptimal results, as the initial stage can absorb local deformations, biasing the residual passed to the diffeomorphic registration. To address this, we introduce a Joint Affine-Diffeomorphic framework, based on the large deformations model, that estimates both global affine and local diffeomorphic motions simultaneously within a single optimization. We propose two models: a Full Affine (FA) model that combines affine and diffeomorphic deformations, and a Decomposed Affine (DA) model that restricts the affine part from FA to rotations, translations, and anisotropic scalings. To numerically implement these models for image registration tasks, we develop a tailored optimization strategy that combines progressive affine enrichment, gradually increasing the complexity of the affine component, with a variational weighting scheme that smoothly manages the coarse-to-fine handover between the affine and diffeomorphic components. Evaluated on 2D synthetic datasets and 3D brain MRIs from the IXI cohort, our unsupervised approach avoids the pathological deformations of sequential baselines. We demonstrate that our joint formulation outperforms in Dice overlap two state-of-the-art deep learning foundation models, CARL and uniGradI-CON, as well as a sequential baseline using FLIRT for the classical affine registration followed by LDDMM. Our implementation is publicly available.

==> sections/99_old_constraints.tex <==


% By theory reduction \cite{MARSDEN1974121}, we can decouple the actions of affine motions and diffeomorphisms by the introduction of constraints on $(I,p^I) \in T^*\mathcal{I}$. These constraints arises from symmetries in the Hamiltonian. In our framework, such symmetries occur when the space of vector fields $V$ is invariant under the action of rotations and translation, as in the case for a Gaussian RKHS. Nevertheless, we are not able to directly apply reduction method since the transport of images by affine deformations is not exactly an action unless the support is small enough, as explained in \cref{prop:transport_support}. However, we can still define constraints on covectors
% \begin{empheq}[left=\empheqlbrace]{align}
%     & \operatorname{Skew}\left[p^AA^{\top} - A^{\top}p^A + p^b b^{\top}  - \int_{\Omega}\tilde{p}^I(x) \nabla \tilde{I}(x) x^\top dx\right] = 0 \tag{$C_{I,1}$} \label{eq:constraints_rot} \\
%     &\int_{\Omega} \tilde{p}^I(x) \nabla \tilde{I}(x) dx = 0 \tag{$C_{I,2}$} \label{eq:constraints_trans}
% \end{empheq}
% where, for any matrix $M\in \R^{d\times d}$, the element $\operatorname{Skew}(M)=\frac{1}{2}(M-M^{\top})$ is the skew-symmetric part of $M$.
% The first constraint represents the affine momentum, while the second corresponds to the translation momentum. Enforcing these conditions ensures a decoupling between the diffeomorphic deformation and the global translations and rotations deformations. We will verify, through an explicit computation and under some assumptions that we will specify, a variant of Noether's theorem adapted to our setting.
% \begin{proposition}[Constraints conservation] Let $\left((\tilde{A}_t,\tilde{b}_t,I_t),(p^A_t,p^b_t,p_t^I)\right)$ satisfy the Hamiltonian equations given in \cref{prop:geod_eq_decoupled}. Suppose also that $\operatorname{Supp}(I_0) \subset \Omega$, then the constraints \eqref{eq:constraints_rot} and \eqref{eq:constraints_trans} are conserved during the dynamic.
% \end{proposition}
% \begin{proof}
% Let us denote $h_t(x) = \tilde{p}_t^I(x) \nabla \tilde{I}_t(x)$ and $\tilde{v}_t(x) = \tilde{A}_t^{-1}v_t(\tilde{A}_t x+\tilde{b}_t)$ such that the dynamical equation of $\tilde{I}$ and $\tilde{p}^I$ can be rewritten as:\begin{equation}
%     \dot{P}_t = - \int_{\Omega} (d \tilde{v}_t(x))^\top h_t(x) dx.
% \end{equation}
% By definition of $\tilde{v}_t$, its Jacobian is $d \tilde{v}_t(x) = \tilde{A}_t^{-1} d v_t(\tilde{A}_t x + \tilde{b}_t) \tilde{A}_t$, which implies $(d \tilde{v}_t(x))^\top = \tilde{A}_t^\top d v_t(\tilde{A}_t x + \tilde{b}_t)^\top \tilde{A}_t^{-\top}$. 
% Let us perform the change of variables $y = \tilde{A}_t x + \tilde{b}_t$, and the associated variable $\hat{h}_t(y) = \frac{1}{\det(\tilde{A}_t)} \tilde{A}_t^{-\top} h_t(\tilde{A}_t^{-1}(y - \tilde{b}_t))$. The time derivative becomes:
% \begin{equation}
%     \dot{P}_t = - \tilde{A}_t^\top \int_{\Omega} d v_t(y)^\top \hat{h}_t(y) dy.
% \end{equation}
% Recall that the optimal condition on the diffeomorphic vector field is given by $v_t = - K_V(\hat{h}_t)$. Since the Gaussian kernel is radial, its spatial derivative is anti-symmetric ($\nabla_x k_V(x,y) = - \nabla_y k_V(x,y)$), guaranteeing that $\int_{\Omega} d v_t(y)^\top \hat{h}_t(y) dy = 0$.
% Consequently, $\dot{P}_t = 0$. 

% \end{proof}

% However, the second condition \ref{eq:constraints_rot} is not conserved during the dynamic. Indeed, by denoting $L_t = \int_{\Omega} h_t(x) x^\top dx$, the angular momentum corresponds to its anti-symmetric part $J_t = \int_{\Omega} \tilde{p}^I(x) (\nabla \tilde{I}(x) x^\top - x \nabla \tilde{I}(x)^\top)dx=L_t - L_t^\top$. Using the same integration by parts strategy as in the previous proof, we obtain:
% \begin{equation}
%     \dot{L}_t = \int_{\Omega} h_t(x) \tilde{v}_t(x)^\top dx - \int_{\Omega} (d \tilde{v}_t(x))^\top h_t(x) x^\top dx.
% \end{equation}
% Applying the same change of variables $y = \tilde{A}_t x + \tilde{b}_t$ to both terms, and noting that $x^\top = (y^\top - \tilde{b}_t^\top) \tilde{A}_t^{-\top}$, we get:
% \begin{align*}
%     \dot{L}_t &= \tilde{A}_t^\top \left( \int_{\Omega} \hat{h}_t(y) v_t(y)^\top dy \right) \tilde{A}_t^{-\top} \\
%     &\quad - \tilde{A}_t^\top \left( \int_{\Omega} d v_t(y)^\top \hat{h}_t(y) (y^\top - \tilde{b}_t^\top) dy \right) \tilde{A}_t^{-\top}.
% \end{align*}
% First, since the condition on translation vanishes $P_t = \int_{\Omega} (d \tilde{v}_t(x))^\top h_t(x) dx=0$, it follows that
% $\left( \int_{\Omega} d v_t^\top \hat{h}_t dy  \right)\tilde{b}_t^\top= 0$. Then, the expression simplifies to
% \begin{equation}
%     \dot{L}_t = \tilde{A}_t^\top S_t \tilde{A}_t^{-\top} \quad \text{where} \quad S_t = \int_{\Omega} \Big( \hat{h}_t(y) v_t(y)^\top - d v_t(y)^\top \hat{h}_t(y) y^\top \Big) dy.
% \end{equation}
% since the matrix $S_t$ is symmetric due to kernel properties.
% Then, the evolution of $J_t$ is given by:
% \begin{equation}
%     \dot{J}_t = \dot{L}_t - \dot{L}_t^\top = \tilde{A}_t^\top S_t \tilde{A}_t^{-\top} - \tilde{A}_t^{-1} S_t \tilde{A}_t.
% \end{equation}
% Even though $S_t$ is symmetric, the conjugated matrix $\tilde{A}_t^\top S_t \tilde{A}_t^{-\top}$ is generally not symmetric unless $\tilde{A}_t$ is constrained to be a scaled rotation matrix (where $\tilde{A}_t^\top \propto \tilde{A}_t^{-1}$). 
% As a result, $\dot{J}_t \neq 0$ and the constraint \ref{eq:constraints_rot} is not conserved. However, in the context of geodesic shooting, enforcing this constraint is only strictly required on the initial costate $\tilde{p}^I_0$. Then, to perform matching while decoupling diffeomorphic and global rotations and translations deformations, it is sufficient to enforce constraints \ref{eq:constraints_rot} and \ref{eq:constraints_trans} at time $t=0$.

% \end{proof}


% If the Hilbert space $V$ generating the vector fields is invariant by the action of rotations and translations (for example with a Gaussian RKHS), the Hamiltonian exhibits natural symmetries. We cannot directly apply Noether's theorem or standard symplectic reduction since the transport of images by rotations and translations only is a valid group action when the support of images is sufficiently small, as discussed previously. Nevertheless, we can still explicitly define constraints on covectors, as established in  \ref{sec:aff_match_problem}
% \begin{equation}
% \label{constraints_images}
% \tag{$C_I$}
% \left\{
%     \begin{array}{l}
%         \int_{\Omega} p^I(x) (\nabla I(x) x^\top - x \nabla I(x)^\top) dx = 0\\
%         \int_{\Omega} p^I(x) \nabla I(x) dx = 0
%     \end{array} 
%     \right.
% \end{equation}
% The first constraint corresponds to the angular momentum, and the second to the translation momentum. Enforcing these constraints on the costate $p^I$ ensures that the diffeomorphism does not act as a rotation or translation on the image, performing as a decoupling between actions of $\D{\alpha}-Isom(\R^d)$ and $\Diff_{C_0^k}(\R^d)$ on the image. In what follows, we will demonstrate a variant of Noether's theorem adapted to our setting.
% \begin{proposition}[Constraints conservation] Let $\left((\alpha_t,R_t,T_t,I_t),(p^s_t,p^A_t,p^b_t,p_t^I)\right)$ satisfy the Hamiltonian equations in \cref{prop:geod_eq_scal_isom}. Suppose also that $\operatorname{Supp}(I_0) \subset \Omega$, then the constraints \eqref{constraints_images} are conserved during the dynamic.
% \end{proposition}

% \begin{proof}
%     Let introduce the flow $\varphi_t$ of $v_t$, i.e. satisfying $\dot{\varphi}_t=v_t\circ\varphi_t$, with initial condition $\varphi_0=\id$. Since $I_S\in H^1(\Omega,\R)$, and as stated in proposition \ref{flow_images}, we get that 
%     \[
%     I_t=I_S\circ \varphi_t^{-1}.
%     \]
%     Similarly the covector $p^I_t$ satisfies the integrated formulation
%     \[
%     p^I_t = p^I_0\circ\varphi_t^{-1}\lvert d\varphi^{-1}_t\rvert
%     \]
%     which corresponds to the cotangent lift of the action of $\varphi_t$ on $p^I_0$. We can now prove that the first constraint (corresponding to the angular momentum) is conserved. Recall the notation of the skew-symmetric mapping $\operatorname{Skew}:M_d(\R)\to \mathfrak{so}_d$, $\operatorname{Skew}(M) =\frac{1}{2}(M-M^\top)$ so that 
%     \[
%         \frac{1}{2}\int_{\Omega} p_t^I(x) (\nabla I_t(x) x^\top - x \nabla I_t(x)^\top) dx = \operatorname{Skew}\left(\int_\Omega p^I_t(x) \nabla I_t(x)x^\top dx\right)\\
%     \]
%     Moreover, using the change of variable induced by $\varphi_t^{-1}$, we see that 
%     \begin{align*}
%       \operatorname{Skew}\left(\int_\Omega p^I_t(x) \nabla I_t(x)x^\top dx\right) = \operatorname{Skew}\left(\int_\Omega p^I_0(x)\,d\varphi_t(x)^{-\top}\nabla I_S(x)\varphi_t(x)^\top dx\right)  
%     \end{align*}
%     This equality allows to reinterpret the constraint as the angular momenta of the particles $\varphi_t(x)$ with covectors $p^I_0(x)\,d\varphi_t(x)^{-\top}\nabla I_S(x)$. By derivating this expression, we then get
%     \begin{align*}
%         \frac{d}{dt}\operatorname{Skew}\left(\int_\Omega p^I_t(x) \nabla I_t(x)x^\top dx\right) &= \frac{d}{dt}\operatorname{Skew}\left(\int_\Omega p^I_0(x)\,d\varphi_t(x)^{-\top}\nabla I_S(x)\varphi_t(x)^\top dx\right) \\
%         &= \operatorname{Skew}\left(-\int_\Omega p^I_0(x)\,dv_t(\varphi_t(x))^\top d\varphi_t(x)^{-\top}\nabla I_S(x)\varphi_t(x)^\top dx\right)  \\  &+ \operatorname{Skew}\left(\int_\Omega p^I_0(x)\,d\varphi_t(x)^{-\top}\nabla I_S(x)\left(v_t\circ\varphi_t(x)\right)^\top dx \right) \\
%     \end{align*}
%     We recall that the condition on the controls in \ref{prop:geod_eq_scal_isom} gives that
%     \[
%     v_t(x) = -\int_\Omega k_\sigma(x,y)p^I_t(y)\nabla I_t(y) dy = -\int_\Omega k_\sigma(x,\varphi_t(y))p^I_0(y)d\varphi_t(y)^{-\top}\nabla I_S(y) dy
%     \]
%     so that the first term of the previous integral becomes
%     \begin{align*}
%         \operatorname{Skew}&\left(-\int_\Omega p^I_0(x)\,dv_t(\varphi_t(x))^\top  d\varphi_t(x)^{-\top}\nabla I_S(x)\varphi_t(x)^\top dx\right)   \\ &=\operatorname{Skew}\left(\int_\Omega\int_\Omega p^I_0(x) p^I_0(y)\nabla_1k_\sigma\left(\varphi_t(x),\varphi_t(y)\right) \left\langle d\varphi_t(y)^{-\top}\nabla I_S(y), d\varphi_t(x)^{-\top}\nabla I_S(x)\right\rangle \varphi_t(x)^\top dx \right) \\
%         &= \operatorname{Skew}\left(\int_\Omega\int_\Omega \left\langle \tilde{p}_t(x), \tilde{p}_t(y)\right\rangle \nabla_1k_\sigma\left(\varphi_t(x),\varphi_t(y)\right) \varphi_t(x)^\top dx \right)
%     \end{align*}
%     where $\tilde{p}_t(x)= p^I_0(x)d\varphi_t(x)^{-\top}\nabla I_S(x)$. Since the kernel $k_\sigma$ is invariant by rotation, this means in particular that 
%     \[
%     \nabla_1k_\sigma\left(\varphi_t(x),\varphi_t(y)\right) \varphi_t(x)^\top = - \nabla_1k_\sigma\left(\varphi_t(y),\varphi_t(x)\right) \varphi_t(x)^\top
%     \]
%     and we get then that the first term $ \operatorname{Skew}\left(\int_\Omega p^I_0(x)\,dv_t(\varphi_t(x))^\top  d\varphi_t(x)^{-\top}\nabla I_S(x)\varphi_t(x)^\top dx\right)$ is equal to $0$. Similarly for the second term, we have
%     \begin{align*}
%         & \operatorname{Skew}\left(\int_\Omega p^I_0(x)\,d\varphi_t(x)^{-\top}\nabla I_S(x)\left(v_t\circ\varphi_t(x)\right)^\top dx \right) \\
%         &=-\operatorname{Skew}\left(\int_\Omega\int_\Omega p^I_0(x)\,d\varphi_t(x)^{-\top}\nabla I_S(x) k_\sigma\left(\varphi_t(x),\varphi_t(y)\right)p^I_0(y) \left(d\varphi_t(y)^{-\top}\nabla I_S(y)\right)^\top dx \right) \\
%         &= -\operatorname{Skew}\left(\int_\Omega\int_\Omega k_\sigma\left(\varphi_t(x),\varphi_t(y)\right) \tilde{p}_t(x) \tilde{p}_t(y)^\top dx \right)\\
%         &= 0.
%     \end{align*}
%     Therefore, we finally conclude that angular momentum is conserved, i.e.
%     \[
%     \frac{d}{dt}\operatorname{Skew}\left(\int_\Omega p^I_t(x) \nabla I_t(x)x^\top dx\right)=0
%     \]
%     The conservation of the second constraint, corresponding to the translation momentum can be proved the same way using the change of variable induced by $\varphi_t$. It is actually easier to prove it using Stokes theorem directly :
%     \begin{align*}
%         \frac{d}{dt}\int_\Omega p^I_t(x)\nabla I_t(x)dx &= -\int_\Omega \nabla\cdot (v_tp^I_t)(x)\nabla I_t(x)dx - \int_\Omega p^I_t(x)\nabla \langle\nabla I_t(x), v_t(x) \rangle dx\\
%         &= -\int_\Omega \nabla\cdot (v_tp^I_t)(x)\nabla I_t(x)dx + \int_\Omega \nabla p^I_t(x) \langle\nabla I_t(x), v_t(x) \rangle dx\\
%         &= -\int_\Omega \left((\nabla\cdot v_t(x))p^I_t(x)+ \langle v_t(x),\nabla p^I_t(x) \rangle\right)\nabla I_t(x) dx+ \int_\Omega \nabla p^I_t(x) \langle\nabla I_t(x), v_t(x) \rangle dx\\
%         &= \int_\Omega\int_\Omega \nabla\cdot \left(k_\sigma(.,y)p^I_t(y)\nabla I_t(y)\right)(x) p^I_t(x)\nabla I_t(x) dxdy \\
%         &= \int_\Omega\int_\Omega \nabla_1k_\sigma(x,y)p^I_t(y)\nabla I_t(y) p^I_t(x)\nabla I_t(x) dxdy \\
%         &= 0.
%     \end{align*}
    
% \end{proof}
